Multi-Model 3D Registration: Finding Multiple Moving Objects in Cluttered Point Clouds

We investigate a variation of the 3D registration problem, named multi-model 3D registration. In the multi-model registration problem, we are given two point clouds picturing a set of objects at different poses (and possibly including points belonging to the background) and we want to simultaneously reconstruct how all objects moved between the two point clouds. This setup generalizes standard 3D registration where one wants to reconstruct a single pose, e.g., the motion of the sensor picturing a static scene. Moreover, it provides a mathematically grounded formulation for relevant robotics applications, e.g., where a depth sensor onboard a robot perceives a dynamic scene and has the goal of estimating its own motion (from the static portion of the scene) while simultaneously recovering the motion of all dynamic objects. We assume a correspondence-based setup where we have putative matches between the two point clouds and consider the practical case where these correspondences are plagued with outliers. We then propose a simple approach based on Expectation-Maximization (EM) and establish theoretical conditions under which the EM approach converges to the ground truth. We evaluate the approach in simulated and real datasets ranging from table-top scenes to self-driving scenarios and demonstrate its effectiveness when combined with state-of-the-art scene flow methods to establish dense correspondences.

==> references/preamble_algo.tex <==
%!TEX root = main.tex
\lstdefinelanguage{mine} 
{morekeywords={while,True,if,break,=,return,function,for,until,in,input,output,assumptions,assumption,invariant,loop,variant,end,invariant,precondition,variables}, 
sensitive=false, 
morecomment=[l]{\#}, 
morecomment=[il]\%{.}, 
morecomment=[s]{/*}{*/}, 
morestring=[b]", 
} 

\lstset{% general command to set parameter(s) 
basicstyle=\small\rmfamily, % print whole listing small 
keywordstyle=\color{black}\bfseries, 
% underlined bold black keywords 
identifierstyle=, % nothing happens 
commentstyle=\color[rgb]{0.2,0.2,0.2},
stringstyle=\ttfamily, % typewriter type for strings 
showstringspaces=false,
mathescape=true,
fontadjust=true,
columns=fullflexible} % no special string spaces 
\lstset{frameround=fttt,frame=none}

\usepackage{calc}
\newlength\listingnumberwidth
\setlength\listingnumberwidth{\widthof{00}}
\lstset{
numbers=left,
xleftmargin=\listingnumberwidth,
numbersep=1em
}


\lstset{escapeinside={*@}{@*}}

\newcommand{\tuple}[2]{\langle#1,#2\rangle}

==> tex/alg.tex <==
%!TEX root = ../main.tex

\begin{algorithm}[t]
\caption{Expectation-Maximization (EM)}
\label{alg:EM}
\SetAlgoLined
\small
\begin{algorithmic}[1]
\STATE \textbf{Input:}
 Point clouds $S := \{(\va_i,\vb_i)\}_{i=1}^n$,
Initial clusters $\cH := \{H_j \subset S \mid j \in [K] \}$, 
Threshold $\tau$, 
Number of iterations $T$,
Minimum cluster size $m_{\min}$
% \vspace{1mm}
% \STATE 
% Define the following: \\
% Initial assignment: For $\vp \in S$, $\alpha(\vp) := i$ where $\vp \in H_i$. \\
% Initial weighted likelihood: $W_{i,j; \infty}^{(0)} := 1$ \\
\smallskip

\FOR{$r \in [T]$}

\STATE {\color{gray} \% Compute a pose, weight, and variance for each cluster}
\FOR{$j \in [K]$}
% \STATE Remove those hypotheses with very few samples assigned to them, and update the rest via Horn's method.
% \vspace{3mm}

\STATE $(\MR_j^{(r)}, \vt_j^{(r)}) := \text{Horn}(H_j)$. \label{line:procrustes} \\
\STATE  $\pi_j^{(r)} := |H_j|/n$. \label{line:weight} \\
% |H_i|/m
% \text{This is initially the size of cluster $k$ over total sample size.}\\
% \text{$E_j$ denotes the following set of errors} 
\STATE  $E_{j} := \{ \vb - \MR_j^{(r)} \va - \vt_j^{(r)} \mid (\va, \vb) \in H_j \}$\\
 \STATE $\sigma_j^{(r)} := \sqrt{ \frac{1}{3} \trace{ \text{cov}(E_j) }}$ \label{line:variance} 
%\sqrt{ (1/3)\sum_{q=1}^3 \textit{Var}(E_j \cdot e_q) }$
\ENDFOR
\smallskip
\textbf{E-step:}\\
\smallskip
% \vspace{3mm}
\FOR{$j \in [K]$ and $i \in [n]$}  
% \STATE Estimate the weighted likelihood:
\STATE    $ W_{i,j; \tau}^{(r)}$ := eq.~\eqref{eq:likelihood}
    %\text{Likelihood}(\MR_j^{(r)},\vt_j^{(r)},\sigma_j^{(r)},\va_i,\vb_i,\tau)$
% \STATE where $\pi_j$ is the weight for hypothesis; $\phi_j(\vb_i|\va_i)$ denotes the independent multivariate Gaussian density of $\vb_i$ for mixture $j$ with $h_j(\va_i)$ as mean and $\sigma_k^2 I_3$ as covariance. 
\ENDFOR
% of $\vb_j$ being generated from $\va_j$ using the hypothesis $h_i$, 
% when the noise is Gaussian with standard deviation $\sigma$. 
% Here $\phi_\sigma(\cdot)$ is the PDF of a Gaussian distribution with variance $\sigma^2$.\\
\smallskip
\STATE {\color{gray} \% Remove small clusters $H_j$ from $\cH$}
\FOR{$j \in [K]$}
\IF{$|H_j| < m_{\min}$} 
\STATE remove cluster $j$ from $\calH, \pi_j^{(r)}, \sigma_j^{(r)}, W_{i,j; \tau}^{(r)}$
\STATE $K := K - 1$ 
\ENDIF
\ENDFOR
\smallskip
\textbf{M-Step:}\\
\smallskip
\STATE {\color{gray} \% Update clusters} %  $\vtheta_i^{(r)}$
\FOR{ $i \in [n]$}
\STATE if $j^\star = \argmax_{j \in [k]} W^{(r)}_{i, j;\tau}$, add $(\va_i, \vb_i)$ to cluster $H_{j^\star}$
%$\alpha^{(r)}((\va_i, \vb_i)) := \argmax_{j \in [k]} W^{(r)}_{i, j;\tau}$.
\ENDFOR
% \STATE Update $\cH$ to be $\{ {\alpha^{(r)}}^{-1}(j) \mid i \in [k] \}$.

\ENDFOR
\RETURN $H_j, \MR_j^{(r)}, \vt_j^{(r)}, \text{ for} j=1,\ldots,K$.
\end{algorithmic}
\vspace{-4mm}
\end{algorithm}

==> tex/problemFormulation.tex <==
%!TEX root = ../main.tex

\section{Problem Formulation}
\label{sec:problemFormulation}

\LC{Luca will take a stab at this}


==> tex/table2.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
\caption{Results for synthetic PASCAL3D+ dataset. Experiment 1: Noiseless. Experiment 2: with additive Gaussian noise. Experiment 3: with additive Gaussian noise and 2 objects with the same motion.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l}
\hline
                    & Metric & \multicolumn{5}{c}{Method}    \\
\cline{3-7}
                    & (Median) & Naive & SRANSAC & T-Linkage         & Ours (Vanilla) & Ours \\
\hline
\hline
\multirow{4}{*}{1}  & Per-point Error [m]    &   0.787 & \textbf{0.0661} &  2.35 &  0.339 & 0.339    \\
                    & Rotation error [deg]     &   6.03e-7 & \textbf{0.0} & 5.96 & \textbf{0.0} & \textbf{0.0}    \\
                    & Translation error [m]  &   5.21e-14 & \textbf{3.44e-14} & 7.34e-14 & 3.55e-14 & \textbf{3.44e-14}    \\
                    & IoU                &   0.603 & \textbf{0.965} & 0.708 & 0.850 & 0.851     \\
\hline
\multirow{4}{*}{2}  & Per-point Error [m]   &   0.181 & 0.457 & 0.359 & 0.0758 &  \textbf{0.0548}     \\
                    & Rotation error [deg]    &   93.4 & 79.8 &  60.5 & 11.1 & \textbf{10.7}    \\
                    & Translation error [m]  &   1.03  & 0.853 & 0.658 & 0.117 & \textbf{0.116}   \\
                    & IoU                &    0.729 & 0.324 & 0.785 & 0.799 & \textbf{0.836}    \\ 
\hline
\multirow{4}{*}{3}  & Per-point Error [m]    & 0.124 & 0.538 & 0.929 &  0.0727 & \textbf{0.0297}   \\
                    & Rotation error [deg]    & 81.8 & 74.7 & 48.9 & 13.3 & \textbf{8.73}     \\
                    & Translation error [m]  & 5.014 & 0.88 & 2.50 &  0.170 &  \textbf{0.154}       \\
                    & IoU                & 0.747 & 0.296 & 0.767 & 0.698 & \textbf{0.874}      \\                                                               
\hline
\end{tabular}
}
\label{table:pascal3d}
\vspace{-6mm}
\end{table}
